Charmonium in a hot, dense medium

In this lecture we apply a thermodynamic Green function formalism developed in the context of nonrelativistic plasma physics for the case of heavy quarkonia states in strongly correlated quark matter. Besides the traditional explanation of charmonium suppresion by Debye screening of the strong interaction, we discuss further effects of relevance when heavy quarkonia states propagate in a medium where strong correlations persist in the form of hadronic resonances. These effects may be absorbed in the definition of a plasma Hamiltonian, which was the main result of this work. This plasma Hamiltonian governs the in-medium modification of the bound state energy levels as well as the lowering of the continuum edge which leads not only to the traditional Mott effect for the dissociation of bound states in a plasma, but can also be applied for a consistent calculation of the in-medium modification of quarkonium dissociation rates.

==> diss-hg.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsubsection{Effective Models in Hadronic Matter} 
%\label{sssec_diss-hg}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
An interesting phenomenological guideline for the present discussion 
is provided by Ref.~\cite{Prorok:2000kv} where the authors show 
that universal $J/\psi$-hadron breakup cross sections with correct
kinematic thresholds but otherwise constant at 3 mb for meson and 5 mb 
for baryon impact are sufficient to explain the observed anomalous 
$J/\psi$ suppression pattern of the NA50 experiment within a multi-component
hadron gas. For a recent update, see \cite{Prorok:2008zm}.
The question arises: How do these assumptions relate to microscopic
calculations of charmonium dissociation reactions in hadronic matter? 
Those can generally be divided into two categories, based on 
hadronic or quark degrees of freedom.
We will primarily review and compare the studies of processes in 
a mesonic medium (predominantly composed of pions and rho mesons) 
within both approaches, including a discussion of in-medium effects. 

Historically, a first calculation of the quark-exchange
reaction, $J/\psi + \pi \to D + \bar{D}^* + c.c.$, was
performed in a nonrelativistic quark model~\cite{Martins:1994hd}
based on applications of the diagrammatic technique developed by
Barnes and Swanson~\cite{Barnes:1991em}
for meson-meson scattering, see also Ref.~\cite{Blaschke:1992qa}.
This calculation showed a strong energy dependence of the cross section
with a peak value of about 6~mb at threshold and a fast decrease due
to a momentum mismatch in the overlap integrals between the meson wave 
functions.
The thermally averaged cross section, which is the relevant quantity for 
estimating the $J/\psi$ dissociation rate, was below 1~mb, roughly in
accordance with phenomenological expectations based on the 
observed suppression in heavy-ion reactions at the SPS.
%
\begin{figure}[!t]
\begin{tabular}{cc}
\includegraphics[width=9cm,height=6.5cm]{bswx_fig1.eps}&
\includegraphics[width=9cm,height=6.5cm]{bswx_fig2.eps}
\end{tabular}
\caption{Born diagrams for quark-exchange processes contributing to
heavy quarkonium dissociation by meson impact (left panels) and the
corresponding cross section for $J/\psi$ breakup by pion impact (right
panel); from Refs.~\cite{Wong:1999zb,Barnes:2003dg}.
Note that in the total cross section also the processes with charge conjugated 
final states are accounted for.
\label{jpsimesondiss}
}
\end{figure}
%
These calculations were extended to other light mesons and excited charmonia
in Refs.~\cite{Wong:1999zb,Barnes:2003dg},
where also more realistic quark-interaction potentials have been used.
In Fig.~\ref{jpsimesondiss} we show the diagrams for
quark-exchange processes at first Born order, which are classified as
``capture'' (C) and ``transfer'' (T) diagrams depending on whether the quark
interaction can be absorbed into the external meson lines; the
latter are to be understood as a resummation of  
ladder-type quark-antiquark interactions.
There are cancellations among the contributions of the different diagrams
due to the small color dipole of the charmonium state. These cancellations
reduce the peak value of the cross section to about 1~mb, as 
also illustrated in Fig.~\ref{jpsimesondiss}.
An open question in this approach is whether the double nature of the pion
-- a Goldstone boson of the broken chiral symmetry and a strongly bound
quark-antiquark -- has a strong influence on these results. 
In the nonrelativistic approach the pion emerges due to a large hyperfine 
splitting in the Fermi-Breit Hamiltonian (as opposed to, e.g., 
instanton-induced interactions), which is not a robust interpretation.
Another question concerns the applicability of the truncation of the 
transfer diagram contributions at the first Born order.
Ladder-type resummations would lead to $s$- and $t$-channel $D$-meson exchange
processes, which are disregarded in the nonrelativistic quark exchange.
Finally, these models are beset with the ``post-prior'' problem due to
the ambiguity in the ordering of quark exchange and interaction lines.

These problems can be resolved within relativistic quark models
developed on the basis of Dyson-Schwinger equations~\cite{Roberts:1994dr} 
for applications to the charmonium dissociation 
problem~\cite{Blaschke:2000zm,Ivanov:2003ge,Bourque:2008es}.
In this approach, the meson-meson interactions are represented by quark-loop
diagrams with three (triangle) and four (box) meson legs. The appearance of
meson-exchange processes can be understood as  a ladder resummation
of quark interaction diagrams in $s$- and $t$-channels, see
Fig.~\ref{jpsipidiss}.
\begin{figure}[!t]
\parbox{10cm}{
\begin{tabular}{ccc}
\includegraphics[width=4.5cm,height=3cm]{Jpsipi-box.eps}&
\includegraphics[width=4.5cm,height=3cm]{DDpi.eps}
\end{tabular}
\\[5mm]
\includegraphics[width=10cm,height=3cm]{psipibox.eps}
}%\hfill
\hspace{-2cm}
\parbox{10cm}{
\includegraphics[width=10cm,height=7.5cm]{sigmatot.new.eps}
}
\caption{Left panel: box and triangle diagrams for meson-meson
interaction vertices contributing to $J/\psi$ breakup by meson impact in
the relativistic quark model~\cite{Blaschke:2000zm} (upper part),
and the origin of $D$-meson exchange from ladder-type resummation (lower part).
Right panel: cross section for pion induced $J/\psi$ dissociation into
open-charm mesons (dotted line) composed of subprocesses with different
final-state $D$-meson pairs: $D+\bar{D}$ (solid), $D+\bar{D}^*$ (dashed),
 $D^*+\bar{D}^*$ (dash-dotted); from Ref.~\cite{Ivanov:2003ge}.
The total cross section includes also the subprocess with $\bar{D}+{D}^*$ 
final state for which the cross section is identical to the charge conjugated 
one (dashed). 
\label{jpsipidiss}
}
\end{figure}
The results for the $J/\psi$ dissociation cross section by pion impact
within the relativistic quark model~\cite{Ivanov:2003ge}, shown in
Fig.~\ref{jpsipidiss}, basically confirm those of the nonrelativistic
approaches~\cite{Martins:1994hd,Wong:1999zb,Barnes:2003dg} shown in 
Fig.~\ref{jpsimesondiss}; residual 
differences may be traced back to the treatment of the transfer-type 
diagrams. In the relativistic treatment these diagrams are resummed beyond the
first Born approximation and result in $D$-meson exchange diagrams which are
absent in the nonrelativistic models. This difference may explain small 
differences in cross section results from both approaches.

Already in 1998, Matinyan and M\"uller~\cite{Matinyan:1998cb} pioneered an
alternative approach to charmonium absorption by light mesons on the basis of
an effective meson Lagrangian, with a local $U$(4) flavor symmetry strongly 
broken by the pseudoscalar and vector meson mass matrices.
This initial  version of the chiral Lagrangian approach gave rather small
cross sections, $\sigma_{\pi\psi}\approx 0.3$~mb at threshold.
It turned out~\cite{Haglin:1999xs,Lin:1999ad} that triple vector-meson 
couplings and contact terms, not included in Ref.~\cite{Matinyan:1998cb},
result in an increase of the breakup cross section by up two orders of 
magnitude, with a rising energy dependence.
A problem for the chiral Lagrangian approaches is the treatment
of hadrons as pointlike objects, which, as usual for an effective theory, 
becomes unreliable at high momentum transfers (due to quark-exchange
substructure effects). The composite nature of hadrons can be accounted
for in an approximate way by vertex form 
factors~\cite{Lin:1999ad,Haglin:2000ar}, which reduce 
the magnitude, and affect the energy dependence, of the cross sections,
see Fig.~\ref{jpsidiss-chiLa}.
%
\begin{figure}[!t]
\begin{tabular}{cr}
\includegraphics[width=7.5cm,height=6cm]{diagrams.eps}&
\includegraphics[width=8.5cm,height=6cm]{sigma-ff.eps}
\end{tabular}
\caption{Feynman diagrams for $J/\psi$ breakup by meson impact
in the chiral Lagrangian approach (left) and the resulting cross sections
for pion- and rho-meson induced processes (right),
from Ref.~\cite{Lin:1999ad,Lin:2002mp}.
Note the role of the form factor at the meson-meson interaction vertices
for the energy dependence and magnitude of the crosss sections.
\label{jpsidiss-chiLa}
}
\end{figure}
%
The choice of the cutoff parameters in the form factors has a 
large effect on the charmonium 
breakup cross sections and remains a matter of 
debate~\cite{Oh:2000qr,Ivanov:2001th,Oh:2002vg,Bourque:2004av}.
Progress may be made by calibrating the form factors with
microscopic approaches as, e.g., the nonrelativistic or
the relativistic quark models \cite{Blaschke:2008mu}.
While the calculations with the relativistic quark model are very cumbersome,
the chiral Lagrangian models offer a very effective tool to assess many 
other dissociation processes required for phenomenology, once the
formfactor question is settled.
In particular, these applications include dissociation processes by nucleon
impact~\cite{Sibirtsev:2000aw,Liu:2001ce} and bottomonium 
dissociation~\cite{Lin:2000ke}.

\begin{figure}[!t]
\parbox{9cm}{
%\begin{tabular}{cc}
\includegraphics[width=8cm,height=4.5cm]{cex.eps}
}\hfill
\parbox{9cm}{
\includegraphics[width=8cm,height=4.5cm]{qQ_ex.eps}
%\end{tabular}
}
\caption{Left panel: Diagrammatic representation of the quark exchange process
contribution to the self-energy~\cite{Blaschke:2000er}; 
right panel: same as left panel but with quark content 
resolved~\cite{Blaschke:2004dv}. 
Three different approaches to the interaction vertex $U_{\rm ex}$ are discussed
in the text and shown in Figs.~\ref{jpsimesondiss}-\ref{jpsidiss-chiLa}.
Diagrams of this type appear in the cluster expansion for two-particle 
properties, see Fig.~\ref{fig:cluster-cluster}.
\label{jpsidiss-diagram}
}
\end{figure}


\begin{figure}[!t]
\parbox{9cm}{
%\begin{tabular}{cc}
%\includegraphics[width=5.5cm,height=4.5cm]{qQ_ex.eps}&
\includegraphics[width=8cm,height=6cm]{P2Sigma_PsiPi.eps}
}\hfill
\parbox{9cm}{
%\includegraphics[width=6cm,height=5cm]{sigmaTPsiRhoNJL.eps}
\includegraphics[width=8cm,height=6cm,angle=0]{SigmaV_PsiPiRho.eps}
%\end{tabular}
}
\caption{Left panel: energy ($s$) and temperature ($T$) 
dependence of the effective cross section ($\sigma^*$) for $J/\psi$ breakup 
by $\rho$-meson impact.
We display $p^2\sigma^*(s;T)$ for better visibility of the effective lowering 
of the breakup threshold when temperatures exceed the $D$-meson Mott 
temperature $T^{\rm Mott}\approx 172$ MeV;
right panel: temperature dependence of the thermally averaged $J/\psi$ 
breakup cross section in a $\pi$-$\rho$ meson gas; 
the calculation with vacuum $D$-mesons (dashed line) is compared to one 
with an in-medium broadening of the $D$-meson spectral function 
(due to the Mott effect at the chiral phase transition) which exhibits
a steplike enhancement (solid line) caused by the effective lowering 
of the breakup threshold; from Ref.~\cite{Blaschke:2002ww}.
\label{jpsidiss-medium}
}
\end{figure}

The energy dependent cross sections for heavy quarkonia
dissociation by hadron impact enable to evaluate the temperature- 
(and density-) dependent dissociation rates in hadronic matter.
Assuming the (short-distance) vertex functions not to be altered by 
the surrounding medium,
there remains the issue of  mass and widths changes
of open-charm hadrons with temperature and density. These, in particular,
imply modifications of the thresholds for the breakup 
processes~\cite{Grandchamp:2003uw,Sibirtsev:1999jr,Tsushima:2000cp,Burau:2000pn,Blaschke:2003ji,Fuchs:2004fh}.
%
In Fig.~\ref{jpsidiss-diagram} we show the diagrammatic representation of 
the quark-exchange contribution to the $J/\psi$ self-energy which develops 
an imaginary part (determining its width or inverse lifetime) due to the 
coupling to open-charm mesons. 
For the interaction vertex $U_{\rm ex}$ three different approaches have been 
discussed above and the corresponding vacuum cross sections are shown in 
Figs.~\ref{jpsimesondiss}-\ref{jpsidiss-chiLa}.
The theoretical basis for the discussion of quark exchange effects to the 
self-energy of heavy quarkonia in strongly correlated quark matter comes from
systematic cluster expansion techniques developed in the context of plasma
physics. For details, see the next subsection and Figs.~\ref{fig:cluster-ex},
\ref{fig:cluster-ex2} and \ref{fig:cluster-cluster}. 
Fig.~\ref{jpsidiss-medium} illustrates the effect of the spectral broadening
of $D$-mesons at the chiral phase transition due to the opening of the 
decay channel into their quark constituents (Mott effect) for temperatures
exceeding the $D$-meson Mott temperature $T^{\rm Mott}\approx 172$ MeV.
Due to an  effective lowering of the  $J/\psi$ breakup threshold the
temperature dependence of the thermally averaged $J/\psi$ 
breakup cross section in a $\pi$-$\rho$ meson gas exhibits a steplike 
enhancement~\cite{Blaschke:2002ww}.
This effect has been discussed as a possible mechanism underlying the
threshold-like anomalous suppression pattern of $J/\psi$'s observed by
the NA50 experiment~\cite{Burau:2000pn,Blaschke:2000er}.


==> intro.tex <==
%Introduction  
The properties of heavy quarkonium states (charmonium and bottomonium)
in a hot and/or dense strongly interacting medium have been intensely 
studied for more than 20 years now, both experimentally and theoretically. 
Current and upcoming heavy-ion collision experiments at the Relativistic 
Heavy-Ion 
Collider (RHIC, at Brookhaven National Laboratory (BNL) in New York), 
at the Large Hadron Collider (LHC, at the European Organization for 
Nuclear Research (CERN) in Geneva) and at the Facility for Antiproton 
and Ion Research (FAIR, at the helmholtz Center for Heavy-Ion Research (GSI) 
at Darmstadt) include heavy quarkonium programs as an essential component 
in their campaigns. The strong interest in heavy quarkonia in medium 
is motivated by their important role in the diagnostics of the highly 
excited medium created in ultrarelativistic heavy-ion collisions.  
A prominent example is the $J/\psi$ suppression effect 
as a possible signal of the formation of a Quark-Gluon Plasma (QGP) 
which was suggested by Matsui and Satz~\cite{Matsui:1986dk} in 1986.
This idea was instrumental in triggering the corresponding experimental 
program at CERN, followed by subsequent campaigns at BNL and the 
future GSI facility. The experimental programs, in turn, have been 
accompanied and pushed forward by a 
broad spectrum of theoretical work (see, e.g., 
Refs.~\cite{Gerschel:1998zi,Vogt:1999cu,Satz:2005hx,Kharzeev:2007ej}). 
After many years of analysis and interpretation of the SPS 
data~\cite{Kluberg:2005yh}, with a first round of RHIC results 
completed and with new insights from the theoretical side
(including thermal lattice theory, effective models and phenomenology),  
it is timely to assess the current state of affairs to help facilitate 
the next stage of developments. 
In the remainder of this introduction we will give an initial view 
on the physics of quarkonia in a hot and dense medium, illustrating some 
of the difficulties in the interpretation of pertinent observables (mostly
charmonia) in heavy-ion collisions at SPS and RHIC. 

\begin{table}[!b]
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline
State ($nL$) & $J^{PC}$ & $m_\Psi$ [MeV] & $\Gamma_{tot}$ [MeV] & $m_\Psi-2m_D$ [MeV] 
\\
\hline  \hline
$\eta_c$ (1$S$)    & $0^{-+}$ & 2980$\pm$1    & 27$\pm$3    &  -750 \\
\hline
$J/\psi$ (1$S$)    & $1^{--}$ & 3097          & 0.093$\pm$0.002 &  -633 \\
\hline
$\chi_{c0}$ (1$P$) & $0^{++}$ & 3415          & 10.2$\pm$0.7    &  -315\\
\hline
$\chi_{c1}$ (1$P$) & $1^{++}$ & 3511          & 0.89$\pm$0.05   &  -219\\
\hline
$h_{c}$ (1$P$)     & $1^{+-}$ & 3526          &     $<$1        &  -204\\
\hline
$\chi_{c2}$ (1$P$) & $2^{++}$ & 3556          & 2.03$\pm$0.12   &  -174\\
\hline
$\eta_c'$ (2$S$)   & $0^{-+}$ & 3637$\pm$4    & 14$\pm$7        &   -92 \\
\hline
$\psi'$ (2$S$)    & $1^{--}$ & 3686           & 0.32$\pm$0.01   &  -44\\
\hline
$\psi''$ (3$S$)   & $1^{--}$ & 3773$\pm$3     & 27.3$\pm$1   &  +43 \\
\hline
\end{tabular}
\end{center}
\caption{Selected properties of $c\bar c$ mesons (generically 
referred to as $\Psi$) in the vacuum, 
as extracted from the recent review of particle physics~\cite{Amsler:2008zzb}.
The particle name in the first column is supplemented by a nonrelativistic
classification of principal quantum number ($n$) and orbital angular
momentum ($L$), the second column gives the total spin, parity and 
charge-conjugation quantum numbers, the third column the meson's mass (errors 
below 1~MeV are not quoted), the fourth column the total decay width, and the 
last column the mass difference to the open-charm threshold (taken as 
2$m_{D^0}$$\simeq$3730~MeV).}
\label{tab_psi-vac}
\end{table}
As a starting point, we collect in Tabs.\ref{tab_psi-vac} and 
\ref{tab_ups-vac} basic properties of the bound-state spectrum of a 
heavy quark ($Q$=$c$,$b$) and its antiquark ($\bar Q$), i.e., 
charmonia and bottomonia, in the vacuum 
(note that the lifetime of the top quark is too short to allow 
for developing a $t\bar t$ bound-state spectrum). These spectra can be 
well understood in terms of a potential-model approach, where the underlying 
potential is of the so-called Cornell-type~\cite{Eichten:1979ms}, 
\begin{equation}
V_{Q\bar Q}(r) = -\frac{4}{3} \frac{\alpha_s}{r} + \sigma r \ ,
\label{Vqq-vac}
\end{equation}
consisting of a (color-) Coulomb term dominant at small $Q$-$\bar Q$ 
separation, $r$, and a linearly rising (``confining") term at 
large $r$. The potential 
description is now understood as a low-energy effective theory of Quantum 
Chromodynamics (QCD) utilizing an expansion in the inverse heavy-quark mass 
($1/m_Q$)~\cite{Bali:2000gf,Brambilla:2004wf}. Moreover, the pertinent 
(vacuum) potential has been computed in lattice QCD~\cite{Kaczmarek:2005ui} 
and found to agree very well with the phenomenological Cornell potential
as deduced from applications to quarkonium spectroscopy.
\begin{table}[!t]
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline
State ($nL$) & $J^{PC}$ & $m_\Psi$ [MeV] & $\Gamma_{tot}$ [MeV] & $m_\Psi-2m_B$ [MeV]
\\
\hline  \hline
%$\eta_c$ (1$S$)    & $0^{-+}$ & 2980$\pm$1    & 27$\pm$3    &  -750 \\
%\hline
$\Upsilon$ (1$S$)    & $1^{--}$ & 9460          & 0.054$\pm$0.001 &  -1100 \\
\hline
$\chi_{b0}$ (1$P$) & $0^{++}$ & 9859          & ?    &  -700 \\
\hline
$\chi_{b1}$ (1$P$) & $1^{++}$ & 9893          & ?   &  -665\\
\hline
%$h_{c}$ (1$P$)     & $1^{+-}$ & 3526          &     $<$1        &  -204\\
%\hline
$\chi_{b2}$ (1$P$) & $2^{++}$ & 9912          & ?   &  -645\\
\hline
%$\eta_c'$ (2$S$)   & $0^{-+}$ & 3638$\pm$4    & 14$\pm$7        &   -92 \\
%\hline
$\Upsilon'$ (2$S$)    & $1^{--}$ & 10023           & 0.032$\pm$0.003  &  -535\\
\hline
$\chi_{b0}$ (2$P$) & $0^{++}$ & 10233          &  ?    &  -325 \\
\hline
$\chi_{b1}$ (2$P$) & $1^{++}$ & 10255          &  ?    &  -305 \\
\hline
$\chi_{b2}$ (2$P$) & $2^{++}$ & 10269          & ?   &  -290\\
\hline
$\Upsilon''$ (3$S$)   & $1^{--}$ & 10355       & 0.020$\pm$0.002  &  -205 \\
\hline
$\Upsilon'''$ (4$S$)  & $1^{--}$ & 10579$\pm$1  & 20.5$\pm$2.5  &  +20 \\
\hline
\end{tabular}
\end{center}
\caption{Same as Table~\ref{tab_psi-vac}, but for low-lying $b\bar b$ mesons
(generically referred to as $\Upsilon$) and an open-bottom threshold of 
2$m_{B^\pm}$$\simeq$10558~MeV (mass differences have been rounded to steps 
in 5~MeV).}
\label{tab_ups-vac}
\end{table}

The good understanding of the vacuum properties of heavy quarkonia in a 
relatively simple framework is one of the reasons why they are believed 
to be a good probe of medium effects. The latter can be roughly categorized
into screening effects in the two-body potential and dissociation reactions 
with constituents of the heat bath. Since the heavy-quark mass is large
compared to the typical temperatures realized in a heavy-ion reaction, 
a further practical benefit emerges: heavy-quark production is believed
to be largely restricted to the earliest phase of the collision, i.e., in 
primordial ``hard"  
(i.e., high-momentum transfer) collisions of the incoming nucleons. On the
one hand, this implies a separation of the (hard) production process
from the subsequent (soft) medium effects, and, on the other hand, it
provides a baseline to determine the initial abundance prior to the formation
of the medium. For total charm production, this picture is consistent with 
current experimental information~\cite{Adler:2004ta,Shahoyan:2007zz} and also 
supported by theoretical estimates~\cite{Levai:1994dx}.
%process which is rather well separated 
%from the soft physics governing the evolution of a potentially formed
%QGP in the subsequent evolution. 

The above setup defines the basic framework to analyze modifications  
in the formation of heavy quarkonia and heavy mesons due to final-state 
interactions induced by the surrounding hot medium in nuclear collisions. 
%The basic principle of their use as indicators
%is similar to the situation in Astrophysics where information about the 
%temperature, density, composition and other properties of stellar atmospheres
%is obtained from an analysis of the modification of emission and absorption
%spectra relative to terrestrial conditions \cite{Kajantie:1985}.
The first and most widely discussed probe in this context is the $J/\psi$.
Somewhat contrary to the expectations at the time, which considered the 
production of charmonium as a primordial plasma 
probe~\cite{Shuryak:1978ij,Cleymans:1984zs}, the suggestion by Matsui and 
Satz~\cite{Matsui:1986dk} asserted that with increasing 
%center-of-mass (cms) energy in 
centrality in a heavy-ion collision a suppression of the $J/\psi$
peak in the dimuon invariant-mass spectrum should occur, relative to the
(Drell-Yan) continuum (which, at sufficiently large invariant mass, is a 
well-established ``hard" process). The underlying mechanism for the
dissociation of the charmonium bound state in a dense medium 
was based on the ``Debye screening" of the binding potential, largely driven
by a deconfinement of color charges and thus intimately connected to
the formation of a QGP. 
The phenomenon itself is, in fact, a rather general one, very similar to the 
dissolution of atomic bound states in electromagnetic plasmas, or to the 
Mott transition in semiconductors~\cite{Mott:1968,Redmer:1997} where 
under high pressure electrons become delocalized and a conduction band emerges,
signaling the plasma state.

Shortly after the prediction of $J/\psi$ suppression, the NA38 experiment 
at the CERN-SPS found evidence for this effect in collisions of 200~AGeV 
oxygen (O) projectiles with uranium (U) nuclei~\cite{Baglin:1990iv}, 
see Fig.~\ref{fig_0-U}. 
\begin{figure}[!t] 
%\epsfysize=9.0cm 
\begin{center}
\begin{minipage}[t]{16.5 cm} 
%\centering\epsfig{file=intro_fig1.epsi,scale=0.8} 
\centering\epsfig{file=intro_fig1.epsi,width=0.8\textwidth}
\end{minipage} 
\caption{First observation of the $J/\psi$ suppression effect in 
O(200~AGeV)-U collisions in the NA38 experiment at CERN-SPS. 
When comparing the invariant-mass spectrum of muon pairs produced 
in peripheral collisions (characterized by a small transverse energy, 
$E_T<34$~GeV; left panel) with that in central collisions 
(at high transverse energy, $E_T>85$~GeV; right panel), a reduction of 
the $J/\psi$ signal relative to the Drell-Yan continuum is apparent 
(figures from Ref.~\cite{Baglin:1990iv}).}
\label{fig_0-U}
\end{center} 
\end{figure} 
\begin{figure}[h] 
%\epsfysize=9.0cm 
\begin{center} 
\begin{minipage}[t]{16.5 cm} 
%\centering\epsfig{file=intro_fig2.epsi,scale=0.8} 
\centering\epsfig{file=intro_fig2.epsi,width=0.8\textwidth} 
\end{minipage} 
\caption{Early comparisons of nuclear-absorption calculations for 
$J/\psi$ suppression to data in $p$-$A$ and $A$-$B$ collisions
with light-ion projectiles~\cite{Gerschel:1993uh}. 
Recent data and analyses are discussed in the main text.}
\label{suppression3}
\end{center} 
\end{figure} 
The interpretation of this observation in terms of QGP formation was 
immediately challenged by more conventional explanations in terms of 
inelastic $J/\psi$ scattering on ``primordial" 
target and projectile nucleons~\cite{Gerschel:1988wn} (i.e., before the
formation of the QGP), as well as on secondary produced hadronic 
``comovers"~\cite{Gavin:1988hs,Vogt:1988fj}.
The systematic experimental analysis of the nuclear mass-number dependence 
of $J/\psi$ production in proton-nucleus ($p$-$A$) collisions at CERN
(NA3~\cite{Badier:1983dg}, NA38~\cite{Baglin:1990iv,Abreu:1998ee}) and 
FNAL (E772~\cite{Alde:1990wa}), as well as in collision systems with
light-ion projectiles (O-U, S-U, O-Cu) at CERN (NA38~\cite{Baglin:1991vb}), 
indeed suggests that the $J/\psi$ suppression in all these experiments can be 
understood in a unified way by the primordial ``nuclear absorption" of the 
charmonium state (with no further reinteractions before being
detected via its dimuon decay). The magnitude of this suppression has 
been characterized by an empirical mean path length, $L$, of the charmonium
traveling through cold nuclear matter at normal density, 
$n_0=0.16$ fm$^{-3}$. The suppression systematics could then be
quantitatively described following the simple absorption law, 
$S_{\rm nucl}=\exp{(-\sigma_{\rm abs}n_0 L)}$ \cite{Gerschel:1993uh},
with the nuclear absorption cross section $\sigma_{\rm abs}$ extracted
from $p$-$A$ collisions\footnote{A more detailed account underlying such 
analysis, based on the Glauber including realistic nuclear density profiles, 
will be given in Sec.~\ref{ssec_nuc-abs} of the main text.}.
%mean path length is determined by the radius, $R_A=1.2~{\rm fm}~A^{1/3}$,
%of the target nucleus as $L_A=\frac{3}{4}R_A$ while for A-B 
%collisions one obtains $L_{AB}=L_A+L_B$. 
In fact, nuclear absorption systematics could not only account for $p$-$A$ 
but also for $A$-$B$ collision systems, see Fig.~\ref{suppression3}, where 
$L=L_A+L_B$ is a schematic measure for the combined path length through 
projectile and target nuclei.
The QGP signal seemingly had vanished~\cite{Gerschel:1993uh}! 
% (as long as the mass numbers are small enough). 

The situation changed when the Pb beam became available at the CERN-SPS.
In central Pb(158~AGeV)-Pb collisions the successor experiment of NA38, 
NA50, found a stronger $J/\psi$ suppression than predicted by the 
extrapolation of the nuclear absorption law (based on the Glauber 
model)~\cite{Gonin:1996wn,Abreu:1997jh}, see Fig.~\ref{anomalous}.
This deviation was dubbed ``anomalous $J/\psi$ suppression", as
opposed to the ``normal suppression" caused by nuclear absorption
(following the simple exponential dependence on the $L$-variable).
A first interpretation of the anomalous suppression as a signal for QGP 
formation was given by Blaizot and Ollitrault~\cite{Blaizot:1996nq} 
within a ``threshold-suppression" scenario. It is based on the 
assumption that a charm-anticharm quark pair cannot hadronize into 
a charmonium state when it is produced in a region where the transverse 
density of participant nucleons exceeds a certain ``critical" value, 
$n_p^{\rm crit}$, see Fig.~\ref{n_part}. This scenario provided a 
consistent explanation of the available data in the sense that the value 
for $n_p^{\rm crit}$ (characterizing the maximal energy density of the
subsequently formed medium) required to describe the suppression in
Pb-Pb was larger than the maximum value $n_p$ reached with light-ion 
projectiles (see also Ref.~\cite{Kharzeev:1996yx}).
\begin{figure}[!htb]
\begin{minipage}{0.5\textwidth}
\includegraphics[width=1.0\textwidth]{anomalous.ps}
\end{minipage}
\hspace{0.5cm}
\begin{minipage}{0.5\textwidth}
\includegraphics[width=.80\textwidth]{anomalous1.epsi}
\end{minipage}
\caption{Anomalous $J/\psi$ suppression in Pb(158~AGeV)-Pb collisions 
at the CERN-SPS measured by the NA50 experiment as a function of the 
Glauber variable $L$ (left panel, from Ref.~\cite{Gonin:1996wn}) and as a
function of the number of charged particles $N_{ch}$ (right panel, from 
Ref.~\cite{Alessandro:2004ap}).
\label{anomalous}
}
\end{figure}
%
\begin{figure}[!htb]
\includegraphics[width=0.8\textwidth,height=8cm]{n_part.eps}
\caption{The transverse density of participants, $n_p$, in S-U 
(left) and Pb-Pb (right) collisions along the direction of the impact 
parameter vector, $\vec b$, for different values of $b=0,2,4,...$fm. 
The dashed line indicates the adopted threshold value 
$n_p^{\rm crit}=3.3$ fm$^{-2}$ for the onset of anomalous $J/\psi$ 
suppression. Figure taken from Ref.~\cite{Blaizot:1996nq}.} 
\label{n_part}
\end{figure}

This initial interpretation was followed by a wide variety of theoretical
investigations including hadronic comover dissociation, parton-induced 
break-up reactions in the QGP, pre-equilibrium effects, and combinations 
thereof. The NA50 collaboration finally concluded that the $J/\psi$
suppression pattern
provides evidence for deconfinement of quarks and gluons~\cite{Abreu:2000ni}
\footnote{For the final NA50 results concerning $J/\psi$ suppression, see
Ref.~\cite{Alessandro:2004ap}}.
One of the controversially discussed issues was (and still is) 
whether the data provide evidence for a ``threshold" or ``onset" 
behavior in terms of step-like patterns in the centrality dependence. 
Further clarification was hoped to be gained from studying intermediate
size collision systems, as recently done by the NA60 
collaboration~\cite{Arnaldi:2006ee,Arnaldi:2007aa}. In In(158~AGeV)-In 
collisions, the ``onset" of anomalous $J/\psi$ suppression does not seem 
to follow 
a scaling with the Glauber variable $L$, but rather with the number of 
participants, $N_{part}$, in the collision. Note that $N_{part}$, 
contrary to $L$, is a quantity closely related to the density of 
secondary particles, eventually forming a QGP, see Fig.~\ref{fig_In-In}.
\begin{figure}[!t] 
%\epsfysize=9.0cm
\begin{center}
\begin{minipage}[t]{16.5 cm}
\centering
%\epsfig{file=intro_fig5.epsi,scale=0.8}
\includegraphics[width=0.85\textwidth]{intro_fig5.epsi}
\end{minipage}
\caption{``Anomalous" $J/\psi$ production (i.e., relative to expectations 
from normal nuclear absorption) in In(158~AGeV)-In collisions
measured by the NA60 experiment compared to 
other projectile-target combinations at the CERN-SPS.
The ``threshold" for anomalous suppression appears to scale with 
the number of participants (right panel) rather than with the Glauber 
variable $L$ (left panel); figures taken from Ref.~\cite{Arnaldi:2006ee}.}
\label{fig_In-In}
\end{center} 
\end{figure} 

%In the context of the CERN summary of the fixed-target heavy-ion program 
%at the SPS in the year 2000,
%, indicating the formation of a new form of matter in Pb(158~AGeV)-Pb 
%collisions, 
In the year 2000 the experimental program at RHIC went underway; first
$J/\psi$ data for Au-Au collisions became available in 
2003~\cite{Adler:2003rc}, while recent ones may be found
in Ref.~\cite{Adare:2006ns}   
Fig.~\ref{fig_phenix} shows the experimental data for $J/\psi$ production
in terms of the so-called nuclear modification factor,
$R_{AA}$, as a function of centrality. It is defined as the yield observed
in a heavy-ion reaction relative to the one in $p$-$p$ 
collisions multiplied
by the number, $N_{\rm coll}$, of binary $N$-$N$ collisions,
\begin{equation}
R_{AA}(N_{part})
=\frac{N_{AA}^{J/\psi}}{\langle N_{coll}\rangle N_{pp}^{J/\psi}} \ .
\end{equation}
In the absence of any suppression (or medium effects) one expects $R_{AA}$=1.
An anomalous suppression of charmonium production was confirmed
in semi-/central Au-Au collisions, with a magnitude  
very similar to the one observed at the SPS. This seems rather surprising 
in view of the factor of 10 higher collision 
energy at RHIC, associated with much higher (initial) energy densities.
However, it had been predicted~\cite{BraunMunzinger:2000px,Thews:2000rj,
Gorenstein:2000ck,Grandchamp:2001pf} that under RHIC and LHC conditions
the copious production of open charm leads to an additional source
of $J/\psi$ production due to the recombination of charm quarks
(or charmed mesons) in the hot and dense medium. Calculations including
both suppression and regeneration mechanisms~\cite{Grandchamp:2001pf}
had predicted that a stronger ``anomalous" suppression is largely 
compensated by secondary production via charm-anticharm
coalescence. This is illustrated in the left panel of Fig.~\ref{fig_phenix}
where a comparison with reaction kinetic models for $J/\psi$
production~\cite{Grandchamp:2003uw,Thews:2005fs} shows that a na\"ive
extrapolation of the concept of an additional ``anomalous"
$J/\psi$ suppression channel in a QGP environment from CERN-SPS to
RHIC fails.
Additional support for the kinetic component of the $J/\psi$ yield at RHIC
follows from the observation that $J/\psi$ suppression is less pronounced
at central rapidity relative to forward rapidity since at central
rapidity the regeneration effect is larger due to a larger charm content
in the medium. On the contrary, dissociation mechanisms should increase the
suppression due to larger energy densities at midrapidity.
\begin{figure}[!t]
\begin{minipage}{0.5\textwidth}
\includegraphics[width=.95\textwidth,height=0.3\textheight]{raa_npart_supp_rapp.eps}
\end{minipage}
\begin{minipage}{0.5\textwidth}
\includegraphics[width=.95\textwidth]{r_aa_n_part_auau_ppg.eps}
\end{minipage}
\caption{$J/\psi$ production, relative to the binary-collision scaled
yield in $p$-$p$ collisions, measured in the PHENIX experiment 
in $\sqrt{s_{NN}}=200~{\rm GeV}$ Au-Au collisions at RHIC.
Left panel: comparison with kinetic 
models~\cite{Grandchamp:2003uw,Thews:2005fs} of charmonium production
at central rapidity, illustrating the importance of secondary 
$J/\psi$ production via charm-anticharm recombination (figure from 
Ref.~\cite{Leitch:2006ff}). 
Right panel: increase of $J/\psi$ suppression at forward relative
to central rapidity,
lending further support to the importance of charmonium regeneration 
mechanisms (from Ref.~\cite{Adare:2006ns}).}
\label{fig_phenix}
\end{figure}

The above discussion has given a first indication of the complexity in
describing and understanding the various facets figuring into quarkonium
observables in heavy-ion collisions,
let alone their interpretation in terms of properties of the
Quark-Gluon Plasma. It is thus mandatory to identify key concepts
and combine them into a comprehensive approach that allows for a systematic 
interpretation of experimental data under a broad range of conditions
(encompassing, e.g., all available collision energies,
from FAIR via SPS and RHIC to LHC). 
This will be the main objective of this article, by means of a critical 
review of existing approaches and their comparison to data. 
%a critical assessment of the
%theoretical and phenomenological al status of charmonium production
%in heavy-ion reactions. In particular, we will try to develop 
%connections between recent theoretical developments and experimental
%observations, and to put together the 
An essential ingredient to such approaches are controlled reference points,
e.g., equilibrium matter for in-medium properties, or $p$-$A$ collisions
to separate ``normal" nuclear effects from hot/dense matter effects.
Our article is roughly organized according to the following decomposition
of the problem: \\
%\begin{itemize}
%\item[(i)]
(1) {\bf Equilibrium properties of charmonia} (Sec.~\ref{sec_equil}): 
these provide the main link
between properties of the QGP and the medium created
in heavy-ion collisions. The basic quantity to be
determined is the thermodynamic spectral function: its pole mass
(binding energy) largely determines the equilibrium abundances (in
connections with the properties of open charm), while in-/elastic
reaction rates determine thermal and chemical relaxation times
and are encoded in the spectral widths. \\
%\item[(ii)] 
(2) {\bf Charmonium transport} (Sec.~\ref{ssec_transport}), 
which is required to evaluate the coupling of the charmonia
to the medium by computing the evolution of their phase space
distribution, starting from realistic initial conditions.
In principle, this evolution progresses toward equilibration,
e.g., as a function of transverse momentum. The method of choice
is a transport treatment incorporating regeneration reactions which
are essential to allow for a relaxation toward thermal and chemical
equilibrium. Since regeneration processes directly draw on open-charm
spectra, a reliable assessment of the latter becomes mandatory. \\
%\item[(iii)]
(3) {\bf Initial spectra and pre-equilibrium interactions} 
(Sec.~\ref{ssec_nuc-abs}): these determine the
initial condition of the transport equation in item (i); they include
modifications relative to spectra in $p$-$p$ collisions ($p_T$ broadening
via Cronin effect, shadowing), as well as absorption and rescattering
on primordial nucleons and secondary particles in the pre-equilibrium
evolution of the medium. \\
%\item[(iv)]
(4) {\bf Observables} (Sec.~\ref{ssec_obs}): to be computed by combining 
all of the above, where as an extra ingredient a realistic modeling of 
the bulk medium evolution is required, ideally (if applicable) in terms 
of a locally thermalized medium if, e.g., within a hydrodynamic evolution, 
or in terms of transport models in (kinetic) regimes of incomplete
thermalization. \\ 
In Sec.~\ref{sec_exp} we give an outlook on the capabilities of, and 
physics questions to be addressed with, future experiments at LHC, RHIC-II 
and FAIR, while Sec.~\ref{sec_sum} contains a brief summary.


%($p_{\rm t}\ge 2$~GeV in the light-quark sector)
%\end{itemize}
%(with emphasis on the first two), augmented by a section on
%theoretical approaches for electromagnetic plasmas and concluded by
%a critical appraisal of presently
%available approaches in comparison to SPS and RHIC data.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 

